Towards Robust Fine-grained Recognition by Maximal Separation of Discriminative Features

Adversarial attacks have been widely studied for general classification tasks, but remain unexplored in the context of fine-grained recognition, where the inter-class similarities facilitate the attacker's task. In this paper, we identify the proximity of the latent representations of different classes in fine-grained recognition networks as a key factor to the success of adversarial attacks. We therefore introduce an attention-based regularization mechanism that maximally separates the discriminative latent features of different classes while minimizing the contribution of the non-discriminative regions to the final class prediction. As evidenced by our experiments, this allows us to significantly improve robustness to adversarial attacks, to the point of matching or even surpassing that of adversarial training, but without requiring access to adversarial samples.

==> figs/intro_cam.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US


\providecommand{\localwidth}{}
\renewcommand{\localwidth}{0.22\linewidth}

\providecommand{\localheight}{}
\renewcommand{\localheight}{3cm}

\begin{figure}[t]
	\footnotesize
	\centering
	\begin{tabular}{cccc}

		\includegraphics[height= \localheight,width=\localwidth]{\Introfig{2492_image_clean_0.jpg}}&
		\includegraphics[height= \localheight,width=\localwidth]{\Introfig{2492_mix_cs_clean.jpg}} &
		\includegraphics[height= \localheight,width=\localwidth]{\Introfig{2492_image_adv_44.jpg}}&
		\includegraphics[height= \localheight,width=\localwidth]{\Introfig{2492_mix_cs_adv.jpg}}\\
		
		
		\includegraphics[height= \localheight,width=\localwidth]{\Introfig{5858_image_clean_0.jpg}}&
		\includegraphics[height= \localheight,width=\localwidth]{\Introfig{5858_mix_cs_clean.jpg}} &
		\includegraphics[height= \localheight,width=\localwidth]{\Introfig{5858_image_adv_2.jpg}}&
		\includegraphics[height= \localheight,width=\localwidth]{\Introfig{5858_mix_cs_adv.jpg}}\\
		
		(a) Clean image & (b) Attention (clean) & (c) Adversarial Image & (d) Attention (adv) \\
		
	\end{tabular}
	\vspace{-3mm}
	\caption{{\bf Visualization of CAMs. on CUB200 dataset}. In the first row,  the network shifts its focus to different regions to misclassifiy to different label. In the second row where the attention regions large remains same but its predicts to its close confusing class of same species which shares the same salient regions such as beak.}
	\label{fig:teaser_CAM}
%\vspace*{-0.4cm}
\end{figure}


==> figs/intro_proto.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US


\providecommand{\localwidth}{}
\renewcommand{\localwidth}{0.15\linewidth}

\providecommand{\localheight}{}
\renewcommand{\localheight}{2cm}

\begin{figure}[t]
	\footnotesize
	\centering
	\begin{tabular}{cccccc}
		
			\includegraphics[height= \localheight,width=\localwidth]{\Introfig{2_original_img.png}}&
		\includegraphics[height= \localheight,width=\localwidth]{\Introfig{2_prototype_activation_map_by_top-1_prototype.png}} &
		\includegraphics[height= \localheight,width=\localwidth]{\Introfig{2_prototype_activation_map_by_top-2_prototype.png}}&
		
		\includegraphics[height= \localheight,width=\localwidth]{\Introfig{3_original_img.png}}&
		\includegraphics[height= \localheight,width=\localwidth]{\Introfig{3_prototype_activation_map_by_top-1_prototype.png}} &
		\includegraphics[height= \localheight,width=\localwidth]{\Introfig{3_prototype_activation_map_by_top-2_prototype.png}}\\

		\includegraphics[height= \localheight,width=\localwidth]{\Introfig{0_original_img.png}}&
		\includegraphics[height= \localheight,width=\localwidth]{\Introfig{0_pre_prototype_activation_map_by_top-1_prototype.png}} &
		\includegraphics[height= \localheight,width=\localwidth]{\Introfig{0_pre_prototype_activation_map_by_top-2_prototype.png}}&

	\includegraphics[height= \localheight,width=\localwidth]{\Introfig{1_original_img.png}}&
	\includegraphics[height= \localheight,width=\localwidth]{\Introfig{1_pre_prototype_activation_map_by_top-1_prototype.png}} &
	\includegraphics[height= \localheight,width=\localwidth]{\Introfig{1_pre_prototype_activation_map_by_top-2_prototype.png}}\\
		
		
		
	
	
		(a) Clean image & (b) top-1   & (c) top-2 & (d) Adversarial  & (e) top-1  & (f) top-2 \\
		 
		
	\end{tabular}
	\vspace{-3mm}
	\caption{{\bf Visualization of activated prototypes}. In the first row for PrototypeNet~\cite{chen2019looks} which ,  we show that the top 2  prototype  activation maps shifts away from those regions of clean samples. However, for our attentional network in the second row, the prototype activation maps remains same even under adversarial attack.}
	\label{fig:teaser_proto}
%\vspace*{-0.4cm}
\end{figure}


==> figs/teaser.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US


\providecommand{\localwidth}{}
\renewcommand{\localwidth}{\linewidth}

\providecommand{\localheight}{}
\renewcommand{\localheight}{5cm}

\begin{figure}[t]
	\footnotesize
	\centering		
		\includegraphics[height= \localheight,width=\localwidth]{\Introfig{teaser.png}}
	\caption{For networks without attention, the prototypes lie closer to each other whereas with our formulation the prototypes from the non-discriminative regions lie close in the feature space and hence confining the subspace of adversary.  
}\label{fig:teaser_tsne}
%\vspace*{-0.4cm}
\end{figure}


==> figs/tsne.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US


\providecommand{\localwidth}{}
\renewcommand{\localwidth}{0.45\linewidth}

\providecommand{\localheight}{}
\renewcommand{\localheight}{5cm}

\begin{figure}[t]
	\footnotesize
	\centering
	\begin{tabular}{ccc}

		\includegraphics[height= \localheight,width=\localwidth]{\Introfig{tsne_proto.png}}&
		\includegraphics[height= \localheight,width=\localwidth]{\Introfig{tsne_ours.png}}\\
		(a) ProtoPNet~\cite{chen2019looks} &  (b) Ours \\
	\end{tabular}
	\vspace{-3mm}
	\caption{{\bf t-SNE visualization of the prototypes from 12 fine-grained classes of the CUB200 dataset.}  In ProtoPNet~\cite{chen2019looks}, the prototypes of different classes are not well separated, making the network vulnerable to attacks. By contrast, our approach yields well-separated discriminative prototypes, while clustering the background ones, which, thanks to our attention module, do not participate the prediction. This complicates the attacker's task. \KN{will add prototype patches in the figures.}}
	\label{fig:teaser_tsne}
%\vspace*{-0.4cm}
\end{figure}


==> tabs/BB.tex <==
\begin{table}[t]
	\centering
	\begin{subtable}[t]{0.48\linewidth}
		\centering
		{\small
			\resizebox{0.97\columnwidth}{!}{%
				 \begin{tabular}{llllllllllll}
					\midrule    
					& \multicolumn{2}{c}{\textbf{VGG16}} &     \multicolumn{2}{c}{\textbf{VGG19} }&      \multicolumn{2}{c}{\textbf{ResNet-34}} \\
					&Clean & AT  & Clean & AT & Clean & AT\\
					\midrule
					AP & &&&&&\\
					AP & &&&&&\\
					AP & &&&&&\\
					AP & &&&&&\\
					\bottomrule
				\end{tabular}		
			}
		}
		\caption{CUB200}
		\label{tab:adaptivepatch_city}
		
	\end{subtable} 
	
	\caption{}
	\label{tab:BB}
\end{table}





==> tabs/Cars_1.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US


%auto-ignore
\begin{table}[t]
\scriptsize
%\begin{small}
  \centering
  \setlength\tabcolsep{6pt}
  \begin{tabular}{c|llllllll}
    \midrule
     Attacks  & Clean & FGSM& FGSM &  BIM  & BIM  & PGD  &  PGD  &  MIM  & MIM\\    
    (Steps,$\epsilon$) &  & (1,2) & (1,8) & (10,2)& (10,8) & (10,2) & (10,8)& (10,2)  & (10,8) \\ 
    \midrule
    \multicolumn{9}{c}{\textbf{VGG16}} \\
    \midrule
    

 
 {AP}~\cite{girdhar2017attentional} &&&&&&&&\\
 \comment{{PNet}~\cite{chen2019looks}&&&&&&&\\
 \textbf{Ours-PNet}&&&&&&&\\
 \textbf{Ours-AP}&&&&&&&\\
 \cmidrule{1-9}
 {AP-AT} &&&&&&&\\
 {PNet-AT}~\cite{chen2019looks}&&&&&&&\\
 \textbf{Ours-PNet-AT}&&&&&&&\\
 \textbf{Ours-AP-AT}&&&&&&&\\
 \midrule
 \multicolumn{9}{c}{\textbf{VGG19}} \\
 \midrule
 {AP} &&&&&&&\\
 {PNet}~\cite{chen2019looks}&&&&&&&\\
 \textbf{Ours-PNet}&&&&&&&\\
 \textbf{Ours-AP}&&&&&&&\\
 \cmidrule{1-9}
 {AP-AT} &&&&&&&\\
 {PNet-AT}&&&&&&&\\
 \textbf{Ours-PNet-AT}&&&&&&&\\
 \textbf{Ours-AP-AT}&&&&&&&\\
 \midrule
 \multicolumn{9}{c}{\textbf{ResNet-34}} \\
 \midrule
 
 {AP} &&&&&&&\\
 {PNet}~\cite{chen2019looks}&&&&&&&\\
 \textbf{Ours-PNet}&&&&&&&\\
 \textbf{Ours-AP}&&&&&&&\\
 \cmidrule{1-9}
 {AP-AT} &&&&&&&\\
 {PNet-AT}&&&&&&&\\
 \textbf{Ours-PNet-AT}&&&&&&&\\
 \textbf{Ours-AP-AT}&&&&&&&\\}
   \bottomrule
  \end{tabular}
  \vspace{1mm}
%\end{small}
  \caption{}
    \label{mnist}
  \label{tab:imagenet}
  \label{cifar10}
\vspace{-7mm}
\end{table}

